Self-supervised Pretraining and Finetuning for Monocular Depth and Visual Odometry

For the task of simultaneous monocular depth and visual odometry estimation, we propose learning self-supervised transformer-based models in two steps. Our first step consists in a generic pretraining to learn 3D geometry, using cross-view completion objective (CroCo), followed by self-supervised finetuning on non-annotated videos. We show that our self-supervised models can reach state-of-the-art performance 'without bells and whistles' using standard components such as visual transformers, dense prediction transformers and adapters. We demonstrate the effectiveness of our proposed method by running evaluations on six benchmark datasets, both static and dynamic, indoor and outdoor, with synthetic and real images. For all datasets, our method outperforms state-of-the-art methods, in particular for depth prediction task.

==> losses.tex <==
%=====================================================
\subsection{Self-supervised Depth Learning} % from SC-Depth
\label{ssec:sc_depth}
In the self-supervised learning framework, a MDE network (depthNet) and a relative 6-DoF camera pose estimation network (PoseNet) are jointly trained on a  number of monocular videos. Given a consecutive frame pair ($I_a,I_b$) randomly sampled from a training video, we predict their depths ($D_a,D_b$) by forwarding the depth network and estimate their relative 6-DoF camera pose $T$ by forwarding the VO branch (PoseNet). 
Then, we generate the warping flow between two images using the predicted depth and pose, followed by synthesizing the $I_a^{'}$ using the flow and $I_b$ via bi-linear interpolation. Finally, we penalize the color inconsistencies between $I_a$ and $I_a^{'}$, and we also constrain the geometry consistency between $D_a$ and $D_b$, which backpropagates the gradients to the networks. The objective function is described below.

First, we use the geometry consistency loss $L_G$ %[1] 
to penalize inconsistencies between $D$ and $D^{'}$ in 3D space
to encourage the predicted depths ($D_a, D_b$) to be consistent with each other in 3D space,
\begin{equation}
L_G = \frac{1}{|{\cal V}|} \sum_{p \in {\cal V}} D_{diff}(p),
\label{eq:lg}
\end{equation}
where $\cal V$ represents valid points that are successfully projected %inside the image. 
from $I_a$ to $I_b$, $D_{diff}$ stands for the pixel-wise depth inconsistency between $D_a$ and $D_b$,
\begin{equation}
D_{diff}(p) = \frac{|D^a_b(p) - D'_b(p)|}{D^a_b(p) + D'_b(p)},
\label{eq:diff}
\end{equation}
To mitigate the influence of moving objects and occlusions
that create geometrical inconsistency across multiple views,
we follow~\cite{bian22csdepthv2} in using the self-discovered mask
%\begin{equation}
$M_s = 1 - D_{diff}$ 
%\label{eq:ddiff} %\end{equation}
which assigns lower weights to dynamics and occlusions than static regions. %since the former is geometrically inconsistent across multiple views. 
%We use this mask in our proposed DRR module( Sec. 3.3) to localize dynamic regions. 

Second, we use the weighted photometric loss $L_P^M$ to constrain the warping flow between $I_a$ and $I_b$ that is generated by the $D_a$ and $T$. Formally,
\begin{equation}
\begin{tabular}{l}
$L_P^M=\frac{1}{|V|} \sum_{p \in V} (M_s(p) \cdot L_P (p))$, \\
$L_P  =\frac{1}{|V|} \sum_{p \in V} (1-\lambda)||I_a(p)-I^{`}_a(p)||_1 + \lambda \frac{1-SSIM_{aa`}(p)}{2})$,\\
\end{tabular}
\label{eq:ssim}
\end{equation}
where $I_a^{'}$ is synthesized from $I_b$ using the warping flow, and SSIM [43] is a widely-used metric to measure image similarity. We set $\lambda$ to 0.85 y following [1].

Third, we use the edge-aware smoothness loss to regularize the predicted depth map. Formally,
\begin{equation}
L_S = \sum_p (e^{-\delta I_a(p)} \cdot \delta D_a(p)^2, 
\label{eq:edge}
\end{equation}
where $\delta$ is the ﬁrst derivative along spatial directions, which guides smoothness by image edges.

The overall objective function is formulated as a weighted sum of the three loss terms above:
\begin{equation}
L_{Self} = L_P^M + \beta L_G + \gamma L_S. 
\label{eq:total}
\end{equation}
where three  $\alpha$ = 1, $\beta$ = 0.5, and $\gamma$ = 0.1 as in [1]. 
%Note that we will replace LS with the proposed normal loss $L_N$ in Sec. 3.4. Moreover, we also use the auto-masking and per-pixel minimum reprojection loss that are proposed in [13] to filter stationary and non-best points during training.

%----------------------------------
%\paragraph{Single-Image Depth Prior}
%Our idea is to leverage the pretrained monocular depth estimation network for generating single-image depth prior, which is then used to boost self-supervised learning. Here we use LeReS~\cite{leres} [25] to generate pseudo-depth, which is trained on large-scale datasets with ground-truth depth labels. Thanks to the supervised training on large-scale data, it shows excellent zero-shot generalization performance on unseen scenes. Note that LeReS was not trained on datasets that we use in this paper for evaluation. An example of LeReS outputs is shown in Fig. 3, where it shows plausible visual results on the DDAD dataset but poor quantitative accuracy. These phenomena echo our motivation, i.e., pseudo-depth is not accurate enough but has potential that can be leveraged for boosting self-supervised learning. More speciﬁcally, we ﬁnd that the good visual results are contributed to several aspects, including (a) correct depth ordinal (nearer/further relation) between objects; (b) excellent smoothness in predicted depth; (c) sharp depth prediction at object boundaries.

%Therefore, based on the above observation, we propose two modules to extract effective supervision signals from pseudo-depth. First, we propose a Dynamic Region Reﬁnement (DDR) module that regularizes self-supervised training with a depth ranking constraint, particularly boosting depth prediction on moving objects. Second, we propose a Local Structure Reﬁnement (LSR) module that constrains the smoothness and object boundaries of the predicted depth. The proposed two modules are presented in Sec. 3.3 and Sec. 3.4, respectively.
